Constraining Gaussian Process Implicit Surfaces for Robot Manipulation via Dataset Refinement

Model-based control faces fundamental challenges in partially-observable environments due to unmodeled obstacles. We propose an online learning and optimization method to identify and avoid unobserved obstacles online. Our method, Constraint Obeying Gaussian Implicit Surfaces (COGIS), infers contact data using a combination of visual input and state tracking, informed by predictions from a nominal dynamics model. We then fit a Gaussian process implicit surface (GPIS) to these data and refine the dataset through a novel method of enforcing constraints on the estimated surface. This allows us to design a Model Predictive Control (MPC) method that leverages the obstacle estimate to complete multiple manipulation tasks. By modeling the environment instead of attempting to directly adapt the dynamics, our method succeeds at both low-dimensional peg-in-hole tasks and high-dimensional deformable object manipulation tasks. Our method succeeds in 10/10 trials vs 1/10 for a baseline on a real-world cable manipulation task under partial observability of the environment.

==> fig/grabber.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[scale=.25]{fig/assets/grabber.png}}
\caption{Our method learns a representation of the obstacle geometry, shown here as a voxel grid. It also provides cost signals that repel the red rope from the obstacle in the direction of the arrows. The blue MPC rollout demonstrates the rope's planned motion out of the previously unknown obstacle as it moves toward the green goal.}
\label{fig:grabber}
\end{figure}

==> fig/heatmap.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[scale=.4]{fig/assets/heatmap.png}}
\caption{Trajectory and surface for the Peg-T task. The modeled obstacle is in purple. The arrows represent GPIS obstacle points and point in the direction of the gradient. Trajectory starts at the green circle and ends at the blue star.}
\label{fig:peg_t}
\end{figure}

==> fig/hook_views.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[scale=.29]{fig/assets/hook_views.png}}
\caption{Multiple views of the same voxelized GPIS. In the upper row, the near side of the hook was visible during task execution and the far side was occluded. In the bottom row, the near side of the hook was occluded and the far side was visible. The arrows show the gradient of the surface.}
\label{fig:hook_views}
\end{figure}

==> fig/hook_visibility.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[scale=.82]{fig/assets/hook_visibility.png}}
\caption{Rope unhooking task. Part of the hook and rope are occluded and the rope starts underneath the hook. The robot is tasked with bringing the center of the rope above the hook.}
\label{fig:hook_visibility}
\end{figure}

==> fig/peg_envs.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[scale=.27]{fig/assets/peg_envs.png}}
\caption{The peg-in-hole environments. Environments and figure are from \cite{TAMPC}.}
\label{fig:peg_envs}
\end{figure}
